Batch Normalization Tells You Which Filter is Important

The goal of filter pruning is to search for unimportant filters to remove in order to make convolutional neural networks (CNNs) efficient without sacrificing the performance in the process. The challenge lies in finding information that can help determine how important or relevant each filter is with respect to the final output of neural networks. In this work, we share our observation that the batch normalization (BN) parameters of pre-trained CNNs can be used to estimate the feature distribution of activation outputs, without processing of training data. Upon observation, we propose a simple yet effective filter pruning method by evaluating the importance of each filter based on the BN parameters of pre-trained CNNs. The experimental results on CIFAR-10 and ImageNet demonstrate that the proposed method can achieve outstanding performance with and without fine-tuning in terms of the trade-off between the accuracy drop and the reduction in computational complexity and number of parameters of pruned networks.

==> main/introduction_backup.tex <==
\section{Introduction}\label{intro}

Deep convolutional neural networks (CNNs) have shown remarkable performance in various computer vision tasks~\cite{long2015fully,Ren2015faster,he2016deep}, however CNNs often require large memory storage and expensive computation costs.
%For instance, ResNet-50~\cite{he2016deep} requires about 25.5M parameters and 4.1G FLOPs (floating point operations) on ImageNet dataset.
Such high demand for memory and computation limits their applications in resource-constrained environment, such as mobile devices.
Among various approaches that tackle this problem, filter pruning approaches have gained attention in recent years for its remarkable reduction of memory storage and computation costs on general tensor processors.



\begin{figure}[t]
\begin{center}
\includegraphics[width=1\linewidth]{latex/figure/figure1/Figure1.pdf}
\end{center}
\begin{center}
\end{center}
\vspace{-0.9cm}
\caption{
Our new finding that the channel importance is already encoded in the pre-trained BN parameters. 
The channels are grouped into \textcolor{red}{high importance (group~1)} and \textcolor{blue}{low importance (group~2)} according to their corresponding BN parameters.
Pruning \textcolor{red}{group~1} results in substantial performance degradation, in contrast to marginal degradation after pruning \textcolor{blue}{group~2}, indicating that the importance of each channel can be determined by its pretrained BN parameters.
The BN parameters is from ResNet-56 trained on CIFAR-10 dataset.
}
\vspace{-0.3cm}
\label{fig:1}
\end{figure}


\iffalse
Among various approaches that tackle this problem, filter pruning approaches have gained attention in recent years due to remarkable reduction of memory storage and computation costs on general tensor processors.
Filter pruning aims to find and remove unimportant filters that do not contribute much to the final output of CNNs.
However, the optimal decision on filter pruning requires intractable computation costs \textendash $\binom{n}{k}$ network feed-forward processes to prune $k$ out of $n$ filters.
Thus, many works have attempted to approximate the optimal filter importance.
\fi

Filter pruning aims to find and remove unimportant filters that contribute the least to the final output by CNNs.
Since the preserved filters after pruning play a crucial role in recovering the final performance~\cite{lin2020hrank}, it is important to identify redundant filters accurately.
From this motivations, several works have attempted to estimate the importance of individual filters.




%잘 프루닝하는게 중요한 이유 -> 파인튜닝 후에도 좋은 성능을 내기 때문
%따라서 제일 중요한 것은 accurate해야 함
%근데 최근 learning based method 들이 filter pruning criterion을 필요로 함
%그래서 availability도 중요하다.




%Among various methods, there have been approaches that try to know where to prune in a pre-trained network.다
%The broadly known approaches are the filter-weight-based methods~\cite{li2017pruning,he2019filter}.
Among these importance estimation methods, the filter-weight-based methods~\cite{li2017pruning,he2019filter}, which determine the importance of filters via the meaningful statistics (\textit{e.g.,} $\ell_1$-norm) of the filter weights, are one of the most widely used approaches.
The prevalence of these methods is mainly due to its simplicity and easy-access property in that they can directly work off-the-shelf on pre-trained networks without relying on data.
For example, several sub-network search methods~\cite{li2020eagleeye,wang2021convolutional} require a filter pruning criterion to prune the full-size pre-trained network according to the searched per-layer pruning ratios and they adopt $\ell_1$-norm criterion due to its easy-access property.
%They achieve such simplicity and accessibility by investigating the meaningful statistics (\textit{e.g.,} $\ell_1$-norm) of the filter weights to determine the importance of filters.
%With the simplicity and the accessibility, the filter-weight-based criteria are utilized by several recent model compression methods \textcolor{red}{how are the criteria used}~\cite{yu2018nisp,huang2017condensenet,he2019asymptotic,he2020learning,li2020eagleeye,wang2021convolutional}.
%With the simplicity and the accessibility, the filter-weight-based criteria are readily available and generalizable to any convolutional network, prompting several recent model compression methods to utilize the criteria within their model compression frameworks~\cite{yu2018nisp,huang2017condensenet,he2019asymptotic,he2020learning,li2020eagleeye,wang2021convolutional}.
%Since the filter-weight-based criteria are readily available and generalizable to any convolutional network, several recent model compression methods utilize these criteria within their model compression frameworks~\cite{yu2018nisp,huang2017condensenet,he2019asymptotic,he2020learning,li2020eagleeye,wang2021convolutional}.
%For example, several sub-network search methods~\cite{li2020eagleeye,wang2021convolutional} require a filter pruning criterion to prune the full-size pre-trained network according to the searched per-layer pruning ratios and they adopt $\ell_1$-norm criterion due to its availability.
%For example, several methods~\cite{li2020eagleeye,wang2021convolutional} adopt a filter pruning criterion to prune a pre-trained network according to the searched per-layer pruning ratios and they adopt $\ell_1$-norm criterion due to its availability.
However, the filter-weight-based methods ignore other operations in CNNs, such as batch normalization~\cite{Ioffe2015batch} and non-linear activation function, which may lead to incorrect filter importance estimation.
%However, there always have been questions on the appropriateness of the filter-weight-based criteria~\cite{ye2018rethinking,molchanov2019importance}.
%and show remarkable reduction of memory storage and computational costs of DCNNs~\cite{yu2018nisp,huang2017condensenet,he2019asymptotic,he2020learning,li2020eagleeye}.

Rather than solely focusing on the filter weight values, the activation-based~\cite{hu2016network,he2017channel, luo2017thinet, lin2020hrank} and gradient-based methods~\cite{molchanov2019importance, molchanov2017pruning} shift the attention to the activation outputs and the gradient values of filter weights, respectively, which have more direct relation to the network performance.
%zhuang2018discirmination,liu2017learning,zhao2019variational,ye2018rethinking,kang2020operation,guo2020dmcp,lin2019towards}
Although these approaches enable relatively accurate filter pruning decisions, they require a number of network feed-forward processes using training data to obtain activation outputs or gradient values.
%Due to these impediments, these data-dependent methods are limited to be used as an off-the-shelf filter pruning criterion.
Due to these impediments, these data-dependent methods are not suitable as off-the-shelf filter pruning criteria.

In this work, we propose a data-independent activation-based filter pruning criterion which achieves the advantages of the aforementioned methods.
In other words, the proposed method does not require any data-dependent computation to find redundant activation channels, which enables simple but accurate filter pruning decisions.
%The proposed method starts from Gaussian assumption on feature values after the batch normalization (BN) layer.
Under the assumption that the output features of batch normalization (BN) layers follow Gaussian distribution, we estimate the per-channel feature distribution after the non-linear activation function and define the importance of each activation channel, and thus the importance of corresponding filter, in terms of BN parameters.


Since the proposed method takes the impact of BN layer and activation functions into account when measuring the filter importance, it can find unimportant filters more accurately with respect to the network final performance than the existing filter-weight-based methods.
Figure~\ref{fig:1} shows that the proposed filter importance can be readily estimated from the BN parameters in a pre-trained network and identifies redundant filters more accurately than the existing filter-weight-based methods.
%To the best of our knowledge, this work is the first to propose an data-independent activation-based filter pruning criterion.

To validate the effectiveness of the proposed method, we conduct extensive experiments on CIFAR-10 and ImageNet dataset with various network architectures.
We show that the proposed criterion can sort the filters in order of importance more accurately than the filter-weight-based methods and even the data-dependent methods, especially on MobileNetV2~\cite{sandler2018mobilenetv2}.
%We experimentally show that when the per-layer pruning ratios are identical, more accurate filter pruning method produces better performance of the pruned network after fine-tuning stage, which shows the importance of accurate filter importance estimation.
%We experimentally show that the less performance drop is after filter pruning, the more accurate the final performance of the pruned network is after fine-tuning, which validates the efficacy of better filter pruning criteria.
Combined with a simple greedy per-layer pruning ratio search strategy, the proposed method also achieves better or competitive results after fine-tuning, compared to the existing complex learning-based pruning methods.

We summarize the contributions of this paper as follows:
%\begin{itemize}[noitemsep,nolistsep]
\begin{itemize}
    %\item To the best of our knowledge, we propose the first off-the-shelf activation-based filter pruning criterion.
    \item Without data-dependent computation, the proposed method estimates per-channel feature distributions after each non-linear activation layer, enabling the measurement of filter importance in terms of the BN parameters.
    \item Experimental results without fine-tuning stages demonstrate that the proposed criterion outperforms the existing filter pruning criteria especially on MobileNetV2.
    %\vspace{0.05cm}
    \item Using a simple greedy per-layer pruning ratio search strategy, we show the proposed criterion can be used to get a compact networks with similar computational efficiency and with better or competitive performance compared to the existing learning-based methods.
\end{itemize}

